MLPerf Power: Benchmarking the Energy Efficiency of Machine Learning Systems from Microwatts to Megawatts for Sustainable AI

Rapid adoption of machine learning (ML) technologies has led to a surge in power consumption across diverse systems, from tiny IoT devices to massive datacenter clusters. Benchmarking the energy efficiency of these systems is crucial for optimization, but presents novel challenges due to the variety of hardware platforms, workload characteristics, and system-level interactions. This paper introduces MLPerf Power, a comprehensive benchmarking methodology with capabilities to evaluate the energy efficiency of ML systems at power levels ranging from microwatts to megawatts. Developed by a consortium of industry professionals from more than 20 organizations, MLPerf Power establishes rules and best practices to ensure comparability across diverse architectures. We use representative workloads from the MLPerf benchmark suite to collect 1,841 reproducible measurements from 60 systems across the entire range of ML deployment scales. Our analysis reveals trade-offs between performance, complexity, and energy efficiency across this wide range of systems, providing actionable insights for designing optimized ML solutions from the smallest edge devices to the largest cloud infrastructures. This work emphasizes the importance of energy efficiency as a key metric in the evaluation and comparison of the ML system, laying the foundation for future research in this critical area. We discuss the implications for developing sustainable AI solutions and standardizing energy efficiency benchmarking for ML systems.

==> tex/archive/methodology.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Overview}
At MLCommons, we have successfully adapted power measurement techniques across various domains, ranging from Tiny Inference to Edge and Datacenter (DC) Inference, as well as HPC and Training Systems. Given the significant diversity in these systems, our approaches vary accordingly. However, the fundamental principles of power measurement remain consistent across all segments.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/power_measurement_method.png}
    \caption{Typical Power Measurement Setup}
    \label{fig:measurement_setup}
\end{figure}


\textbf{Core Concept:}
Any given workload will have multiple phases, namely the initiation phase, the execution phase, and the result assimilation phase. Though end-to-end run time could be an important consideration for overall system performance; from a power measurement perspective, the most critical phase is the execution phase. At MLCommons, we have a philosophy that performance and power are a tuple and that we cannot accurately characterize a system by quoting just one of these two. Energy measurement by definition is the area under the curve (with X-axis being time and Y-axis being Power) and across all of our systems, we aim to measure for the active portion of the workload. As noted, for measuring Energy we would need Power and this is obtained as the product of current drawn by the system and the voltage that is supplied to it. 


\textbf{Metrics of Power Measurement:}
Like performance, power can also be quantified using two different types of metrics - Watts and Energy. Energy is Power multiplied by time. So, when time is of the essence in measuring a benchmark, we measure Energy as the metric for power. When throughput is of the essence for the benchmark, we measure Watts as the metric. For example: Inference per second is a common metric for measuring AI performance. This metric focuses on throughput and when measuring this metric, we report power in Watts. For another scenario, the latency or time-to-train could be the key performance metric that is being tracked. Under these conditions, we would want to measure energy as the metric of choice.

\subsection{MLPerf Tiny Setup and Operation}
The key power-related metric in tiny systems is energy per inference.  Deployed systems will have widely varying latency and throughput requirements, but the impact on battery life due to inference can be easily calculated from the energy required by each inference, expressed in Joules, and the expected inference rate expressed in e.g. frames/sec.  

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/power_measurement_tiny.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/power_measurement_tiny_waveform.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

One concern specific to tiny systems is the possibility of parasitic powering of the SUT.  All commercial integrated circuits include “protection diodes” on the input pins which protect against static discharge or overvoltage events by conducting excess charge to the supply rails.  If the host provides an input voltage higher than the positive supply voltage and that signal is connected to an input, then the protection diodes can deliver power to the positive supply, effectively powering (partially or fully) the SUT from the host.  An effective power measurement system must minimize the risk of accidental corruption of the power measurement. To this end, the Tiny power measurements are performed using an IO Manager that sits between the host and the SUT.  The IO Manager provides a USB connection to the host and connects to the SUT’s UART through an isolating level shifter that is only capable of delivering a negligible	amount of power, thus preventing parasitic powering of the SUT.

Additionally, there is some dead time in the measurement due to communication with the host where the SUT is running but not active on the ML workload.  Energy consumed during this phase should not contribute to the measured energy.  To ensure an accurate measurement, it is important to align the power waveform with the phases of operation performed by the SUT. The SUT toggles a pin to indicate when inference begins and ends.  The energy monitor captures the toggle and relays the timing information to the host, where it is captured by the runner application.

Figure [JH2] shows an energy waveform captured by the runner application.  The x axis is time and the y axis is energy per sample.  Since the sample rate is 1 kS/s, an energy measurement of 70 uJ corresponds to an average power consumption of 70 mW.  Because each pixel in the plot represents multiple samples, the red trace shows the average of all samples represented by a given pixel, while the two gray plots show the minimum and maximum values recorded in the time covered by that pixel.  The gray area from about 90s-130s is one set of inferences, all run on the same input tensor so that the measurement phase is not polluted with extra delay due to communication tasks.  The sum of energy samples during one set of inferences divided by the number of repetitions gives the energy per inference.


\subsection{MLPerf Inference Setup and Operation}
Having reviewed the various systems in the previous sections, we will now delve into a practical example of a power measurement setup that we deploy for the Inference category. To measure the power consumption of a System Under Test (SUT), we implement a client-server type architecture. In this setup, the SUT acts as the client while the server is referred to as the "Director."

We reference Fig. \ref{fig:measurement_setup} for explaining a typical power measurement setup. The SUT is connected to a SPEC-approved power analyzer, which in turn is plugged into a power outlet. The connection between the SUT and the analyzer can be either wired or wireless, depending on available infrastructure. The Director connects to the power analyzer via a wired method, such as USB, Ethernet or GPIB (General Purpose Interface Bus), although some newer standards support wireless communication.

For MLPerf Inference, the director and the SUT initiate a NTP (Network Time Protocol) sync routine to align their timestamp references. The director then initiates communication to the power analyzer through the PTD (Power-Thermal Daemon) API calls. Once the connection is established, the director them sends command the SUT to start executing the loadgen that helps run the workload of interest on the SUT. While the workload is running on the SUT, the director starts logging the power versus time data from the analyzer in a txt file format which is later converted to a csv format for ease of data processing. This file contains the details like current, voltage, phase and power usage of the SUT. While running the workload, the SUT collects the performance log files that timestamp the different phases of executions of the workload. Specifically, the execution phase of the workload will be preceded by a "time start" tag and the conclusion of this phase will have a "time stop" tag. Since the timestamps of the SUT and the director are correlated, the corresponding row items from the power vs time csv file is selected and within this selection, we average the voltages and sum the currents to compute the power of the SUT while executing this workload. This is the reported power along with the reported throughput performance.

\textbf{Enhancing Power Measurement Accuracy Using Ranging:}
Most analyzers are capable of measuring multiple orders of current measurements. Depending on the SUT the analyzer is connected to and the nature of the workload, we could have current that is measured in either amperes or milli/micro amperes. The analyzers trade off sensitivity for range - ie: 1.5A could be the power draw for a particular SUT whereas 0.530 mA could be power draw for another SUT. Since the analyzer is agnostic to the capabilities of the SUT, it has a mode called “Auto Ranging” that performs a sweep when starting to measure current before settling in on a sweet spot of range and accuracy. Depending on the nature of the workload (bursty vs steady state), it could take some time for the analyzer to settle in on this sweet spot. The risk here is that we could lose valuable information if this process takes too long. To address this we do a ranging mode run where the current and voltage levels are initially monitored to observe the maximum ranges they go up to for a particular workload. Once we have this information, we re-run the same workload on the same SUT again, but this time we fix the range of the analyzers to the observed peak value so that we could get higher accuracy within that range.

A note on idle Power Measurement: For MLPerf inference power measurements idle power is not considered separately and is considered part of the inference power usage. So a system with lower idle power is expected to have better inference power efficiency.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/multi_sut_diagram.png}
    \caption{Measurement for Multi-SUT Systems}
    \label{fig:multi_sut}
\end{figure*}

\textbf{Scaling to Multi-Node Inference Setups:}
The above mentioned setup is a typical single-node setup. While scaling to multiple nodes, this setup will need to be adapted both from a hardware and software perspective. Illustrated in Fig. <XX>, we have shown examples of how we can connect multiple analyzers to a single SUT or multiple SUTs to a single analyzer. We currently have a proof of concept working for making such setups work and the plan is to merge this option with the mainline in the coming Inference submissions versions. In all of these variations, the actual current measurement methodology does not change.

% \textbf{Communication and Control:}
% Time to reach the steady state power usage is typically higher than that needed to reach the peak performance. This can be attributed to systems being able to run at peak performance for a while with minimal cooling. As cooling increases, the power usage also increases. (We can use power logs from previous submissions to show that this typically happens after “X” minutes - X should be near 5)
\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/Training_Measurement_Scheme.png}
    \caption{Training and HPC Measurement Methodology Block Diagram}
    \label{fig:training_method}
\end{figure}


\subsection{MLPerf Training and HPC Setup and Operation}
% The homogeneity of the system described above aids in scalability of such a setup and we would be limited by the hardware resources like analyzers, etc. as the system infrastructure scales-out. In many cases, this becomes a serious limiting factor and we need to consider alternative approaches to measuring power. In suhc cases, we would 
Training and HPC clusters for ML training span from single nodes to thousands of nodes consisting of tens of thousands of accelerators.  Many of these clusters are located in secure on-prem datacenters, cloud environments or national labs.  The sheer scale of the machines and their locations and associated security requirements makes the use of separate power analyzers to measure each node and interconnect component practically impossible.  Therefore, a training and HPC-focused methodology was designed to work around these constraints but still adhere to MLPerf's goal of measuring full system power.  
We designed a software-based power measurement scheme that utilizes the existing telemetry infrastructure of large clusters to measure system power. The scheme is flexible enough to handle the diverse range of telemetry systems of different submitters. Figure \ref{fig:training_method} shows a high level block diagram of the training power measurement methodology. 

\subsubsection{Node Level Power Measurement}
For each participating compute node, power measurements should be taken at the node level. This can be achieved using the submitter’s own telemetry systems such as IPMI, RedFish, or iDRAC. To minimize interference with the ML job itself, out-of-band measurement techniques are recommended. Alternatively, power can be measured at the Power Distribution Unit (PDU) level, provided that all nodes supplied by that PDU are involved in the ML job. The accuracy of the telemetry systems used should be thoroughly documented for review.
\subsubsection{Interconnect Power Measurement/Estimation}
For interconnect switches, power can be measured similarly to compute nodes, or an estimated power value can be provided. If estimation is used, the methodology for this estimation must be documented and included in the submission for review.
\subsubsection{Data Logging and Standardization}
Submitters are required to convert their node and interconnect logs to the MLPerf standardized format using the MLPerf Logging Library. This ensures consistency and comparability across different submissions.
\subsubsection{Energy-to-Train Calculation}
Upon submission, the result summarizer parses both performance and power logs together to derive the energy-to-train metric. This involves aggregating the power consumption data over the duration of the ML training process.  The result summarizer determines the ML training process window by extracting the time stamps of the \textit{run\_start} and \textit{run\_stop} log lines in the performance log.  It then parses each node's log file to extract power samples that fall inside the run window.  Energy for each node is calculated by integrating power samples over the run's time window as shown in Algorithm \ref{alg:trnpower}. Total energy is computed by summing the energy across all compute and interconnect components. 

\begin{algorithm}
\caption{Calculate Node Energy}
\label{alg:trnpower}
\KwIn{\textit{run\_start\_time, run\_stop\_time, loglines}}
\KwResult{\textit{agg\_power}}
\SetKw{KwTo}{in}
\SetKw{KwAnd}{and}
\SetKw{KwFrom}{from}
\SetKw{KwReturn}{return}
\textit{prev\_timestamp} $\gets$ \textit{run\_start\_time}\;
\textit{agg\_power} $\gets$ 0\;
\ForEach{\textit{logline} \KwTo \textit{loglines}}{
    \If{\textit{logline.timestamp} $\geq$ \textit{run\_start\_time} \KwAnd \textit{logline.timestamp} $\leq$ \textit{run\_stop\_time}}{
        \If{\textit{logline.key} $=$ \textit{power\_reading}}{
            \textit{agg\_power} $\gets$ \textit{agg\_power} + (\textit{logline.value} $\times$ (\textit{logline.timestamp} - \textit{prev\_timestamp}))\;
            \textit{prev\_timestamp} $\gets$ \textit{logline.timestamp}\;
        }
    }
}
\KwReturn{\textit{agg\_power}}\;
\end{algorithm}

\subsubsection{Submission Process}
Figure \ref{fig:training_method} shows an example block diagram of a hypothetical training cluster. Submitters have two primary options for reporting power measurements:
\begin{itemize}
    \item PDU Measurement: If PDUs are used for power measurement, report the power for pdu\_0 and pdu\_1.
    \item Node Measurement: If out-of-band measurement mechanisms are used, report the power for nodes node\_0:3.
\end{itemize}
The submission process involves the following steps:
\begin{itemize}
    \item Run the benchmark with either of the two node-level telemetry options mentioned above. 
    \item Estimate switch power, if applicable.
    \item Post-process power logs to MLPerf Logging Library format. 
    \item Submit the data in the directory structure specified by the MLPerf Training/HPC rules.
    \item Include documentation on telemetry accuracy and/or interconnect power estimation methodology.
    \item The result summarizer will then process the power logs to compute the total energy consumed during the training process, yielding the energy-to-train metric.
\end{itemize}
By following this methodology, we ensure that power consumption data is accurately captured and standardized, enabling meaningful comparisons across different ML training setups.
% \textbf{Hardware Components}
% \comment{Should this section be moved up, @Tejus need review}
% \begin{enumerate}
%     \item Power Meters: High-precision power meters are used to measure the power consumption of the system. These meters should be capable of measuring power at a fine granularity (e.g., every second or millisecond). MLPerf allows any power analyzers compatible with SPEC PTD but so far most of the MLPerf inference submissions are done using Yokogawa power analyzers
%     \item Data Acquisition System: This system collects power consumption data from the power meters. It is usually a dedicated device running the MLPerf inference power server code and logs power usage over time.
%     \item System Under Test (SUT): This is the hardware platform on which the MLPerf Inference benchmarks will run. It can include CPUs, GPUs, TPUs, or other accelerators.
% \end{enumerate}


% \textbf{Software Components}
% \begin{enumerate}
%     \item Logging Software: MLPerf logger is used to log power consumption data over time. This is needed to synchronize power data with inference performance data.
%     \item Synchronization Tools: The MLPerf Power setup ensures that the power data is timestamped and synchronized with the inference tasks by doing NTP sync at the start of the measurement and a sync check just before the inference starts and immediately after the inference ends.
% \end{enumerate}

% \textbf{Procedure}
% Ranging mode run: In this mode, the actual inference run happens, but without setting a peak current or voltage range to the power analyzer. Here, the power analyzer automatically adjusts the current and voltage levels and determines the peak current and voltage levels for the given inference run on the system.
% Actual power and performance mode run: The peak current and voltage levels determined from the ranging mode run are used to perform the actual power measurement in the testing phase. This ensures that the uncertainty of the measured power is very minimal (? need to add the actual %).
% The ranging mode run is an overhead for power measurement compared to a non-power inference run. Typically this run takes as long as an actual performance run but that is not a strict requirement. We have seen that by doing a 5 minute long ranging mode run, we can determine the peak current and voltage range for the actual test run. (?Add data) (\url{https://docs.google.com/spreadsheets/d/13b4MDUkI-bJFH0qOCPWtmR43vAPy5IM1Ij99L7dgvgo/edit?pli=1&gid=472011955#gid=472011955})

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/image.png}
    \caption{Avg. power variation compared to a full run for different durations of ranging mode runs}
    \label{fig:ranging-mode-variations}
\end{figure}


% \subsection{Power Measurement Setup and Instrumentation}
% \begin{itemize}
%     \item Integration with existing tools
%     \item Training/HPC
%     \begin{itemize}
%         \item Talk about the component level measurement
%         \item Not a clean client-server architecture
%         \item Every component is measured independently
%         \begin{itemize}
%             \item Not orchestrated through a single director
%         \end{itemize}
%         \item Might have to rely on metering tech, which might vary from ``system'' to ``system''
%         \item Trade-off between inclusivity vs. detailed introspection
%         \item Potentially using only a portion of the rack
%         \item Different systems can have slightly different measurement frameworks
%         \begin{itemize}
%             \item Why --
%         \end{itemize}
%     \end{itemize}
%     \item Inference
%     \begin{itemize}
%         \item Correct in a way. For inference, we allow all the SPEC-approved power meters. As of today, all submitters use only Yokogawa. But there are non-Yokogawa SPEC-approved meters as well. It's just that we have not seen many folks adopt that.
%         \item From a framework perspective inference systems will have some consistency
%         \item Instrument the load generator
%     \end{itemize}
% \end{itemize}



% \subsection{Data Collection and Analysis}
% <Not sure we need this section>


% \subsection{Divisions}
% \textbf{Closed}
% \textbf{Open}
% <Does it make sense for this commentary to go here??>



==> tex/archive/results.tex <==
\section{Results/Evaluation}

\comment{We need to define what a result is - I think the current table is showing all model results in a single system as one result}

We have a broad range of MLPerf Power submissions spanning multiple years and several workload versions. Understanding trends in energy efficiency improvements can give insight into industry-wide points of emphasis and comparative trends between workloads and system scales. 

\begin{table}[t!]
\caption{MLPerf Power results submitted per version across inference categories (datacenter, edge, and tiny ML systems) and training systems. Note that power measurement for training was only recently introduced, resulting in fewer submissions for this category compared to the inference category.}
\label{tab:datacenter_corpus}
\centering
\setlength\tabcolsep{2pt} % Reduce horizontal padding
\begin{subtable}[t]{0.23\columnwidth}
    \caption{Datacenter}
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \makecell{Model \\ Version} & \makecell{Total} \\
        \hline
        1.0 & 60 \\
        \hline
        1.1 & 100 \\
        \hline
        2.0 & 146 \\
        \hline
        2.1 & 88 \\
        \hline
        3.0 & 68 \\
        \hline
        3.1 & 56 \\
        \hline
        4.0 & 46 \\
        \hline
        \hline
        Total & 564 \\
        \hline
    \end{tabular}
\end{subtable}%
\begin{subtable}[t]{0.23\columnwidth}
    \caption{Edge}
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \makecell{Model \\ Version} & \makecell{Total} \\
        \hline
        1.0 & 50 \\
        \hline
        1.1 & 94 \\
        \hline
        2.0 & 142 \\
        \hline
        2.1 & 106 \\
        \hline
        3.0 & 189 \\
        \hline
        3.1 & 149 \\
        \hline
        4.0 & 59 \\
        \hline
        \hline
        Total & 789 \\
        \hline
    \end{tabular}
\end{subtable}%
\begin{subtable}[t]{0.23\columnwidth}
    \caption{Tiny}
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \makecell{Model \\ Version} & \makecell{Total} \\
        \hline
        0.5 & 17 \\
        \hline
        0.7 & 26 \\
        \hline
        1.0 & 38 \\
        \hline
        1.1 & 41 \\
        \hline
        1.2 & 18 \\
        \hline
        \hline
        Total & 447 \\
        \hline
    \end{tabular}
\end{subtable}%
\hspace{1em}
\begin{subtable}[t]{0.23\columnwidth}
    \caption{Training}
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \makecell{Model \\ Version} & \makecell{Total} \\
        \hline
        4.0 & 12 \\
        \hline
        \hline
        Total & 12 \\
        \hline
    \end{tabular}
\end{subtable}
\end{table}


\subsection{Energy Efficiency Improvements @Anirban}

%Figure~\ref{fig:mlperf_performance} in Section~\ref{sec:intro} shows the advances in performance of various AI models from December 2018 to June 2024. Older networks such as Mask~R-CNN~\cite{?} and ResNet~\cite{?} show significant early enhancements, followed by stabilization in subsequent years. In contrast, more rennet models, such as GPT-3~\cite{?} and Stable Diffusion~v2~\cite{?}, display notable improvements reflecting recent rapid advancements. BERT-large also exhibits steady progress, with a pronounced increase near the latter part of the timeline. The comparison with Moore's Law cumulative growth highlights that the progress of AI models, particularly GPT-3 and Stable Diffusion, is surpassing conventional hardware advancements, indicating a quicker-than-anticipated development in AI capabilities. 

Figure~\ref{fig:comparison} shows a significant improvement in efficiency in the data center, edge devices, and tiny categories. These advances are quantified in terms of normalized samples per joule, which reflects the growing emphasis on optimizing performance while minimizing energy consumption. The trends indicate substantial progress in making AI more sustainable and scalable in different deployment environments to achieve the performance improvements shown in Figure \ref{fig:mlperf_performance}.

In the data center category, \benchmark{retinanet} shows a significant increase in samples per joule, reaching a peak that is more than three times its original efficiency. Models such as \benchmark{bert-99.0} and \benchmark{resnet} also show consistent progress, with \benchmark{bert-99.0} leveling off between 1.5 and 2.0. \benchmark{gptj-99.0}, meanwhile, shows a notable improvement. This can probably be attributed to the significant attention given to LLM computing efficiency due to its significant impact at scale. Overall, data center models show substantial gains in energy efficiency, with notable improvements in the later iterations.

In the edge category, improvements in energy efficiency are particularly significant. \benchmark{bert-99.0} and \benchmark{rnn-t} are at the forefront with substantial early improvements, reaching up to four times their starting efficiency. In contrast, \benchmark{resnet} exhibits a more steady enhancement, leveling at approximately 1.5 normalized samples per joule. Rapid progress in edge devices underscores the emphasis on refining AI models for real-time, on-device execution, crucial for applications that demand low latency and high energy efficiency.

In the tiny category, we observe significant improvements in efficiency across multiple models. \benchmark{ResNet-V1} and \benchmark{DSCNN} show remarkable progress, both reaching a normalized efficiency of around 100. \benchmark{MobileNetV1 (0.25x)} also demonstrates substantial improvement, achieving a peak of 2 normalized samples per joule. While \benchmark{FC AutoEncoder} shows steady gains, it levels off at a much lower efficiency compared to the other models. These results underscore the rapid advances in AI efficiency for small-scale, resource-constrained environments. In particular, tiny-scale computing has experienced massive improvements in energy efficiency over its early versions, with gains between ~100x and ~1000x across every workload. However, this trend has plateaued since MLPerf-Tiny v1.0, indicating a need for more innovative approaches to continue improving efficiency. Despite individual tiny electronics consuming significantly less power than datacenter or edge devices, improving their energy efficiency remains crucial for the scalability and sustainability of next-generation Internet of Things (IoT) systems.

Overall, the trends across all three categories highlight the ongoing efforts and successes in enhancing AI models' energy efficiency, ensuring that high performance can be achieved sustainably across different environments and use cases.

\subsection{Training Scalability Analysis @Anirban @Hiwot}

As ML models grow in complexity, the time to solution (train) becomes a critical factor in the design of the ML system~\cite{dawnbench}. Researchers and industry practitioners have developed various parallelization strategies to reduce training time by leveraging additional computational resources. However, our MLPerf Power benchmarking reveals that this pursuit of faster training times introduces a new dimension of complexity: energy consumption at scale. To this end, we present a novel analysis of the intricate relationship between system scale, training time, and energy consumption, drawing from our recently released MLPerf Training power benchmarks. 

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/llama70b_finetune_energy_breakdown.png}
\caption{Energy consumption and time-to-train for Llama2-70b LoRA fine-tuning across different numbers of accelerators.}
\label{fig:training_energy_breakdown}
\end{figure}

Figure \ref{fig:training_energy_breakdown} illustrates the time-to-train and energy-consumption metrics from our v1.0 training power submissions for the \benchmark{Llama2-70b} model across three distinct system scales. This data provides crucial insights into the non-linear nature of energy scaling in large-scale ML training systems. Ideally, with perfect parallelization, increasing the number of accelerators should lead to a proportional reduction in training time and linear energy consumption scaling. However, our results reveal a more complex reality. As the system scale increases, we observe diminishing returns in training time reduction. The improvement in training time becomes less pronounced as we add more accelerators, indicating that not all parts of the workload can be perfectly parallelized. Simultaneously, we see non-linear energy consumption growth. The energy required for training increases disproportionately with system scale, primarily due to increased power demands from additional networking infrastructure and other auxiliary components.

These findings underscore the importance of considering energy efficiency alongside performance when designing and deploying large-scale ML training systems. They also highlight the need for a more nuanced approach to system optimization that goes beyond mere parallelization for performance scaling.

Our analysis suggests several key implications for future ML system design. First, architects must carefully consider the energy costs associated with scaling up training systems, which can lead to the development of more energy-efficient accelerators and interconnects. This energy-aware scaling approach is crucial for sustainable AI development. Second, understanding the parallelization characteristics of different ML workloads can help to determine the optimal system scale that balances performance gains with energy efficiency. This workload-specific optimization will be key to maximizing efficiency across various ML tasks. Lastly, future ML systems should optimize not just compute energy, but also other types of energy consumption, such as interconnect energy, which becomes increasingly significant at larger scales. This holistic approach to system design will be essential for truly efficient large-scale ML systems.

As we continue to collect and analyze MLPerf Training power data in future submissions, we aim to define more precise Pareto curves for optimal energy efficiency at various system scales. This ongoing research will provide invaluable guidance to the ML community in designing the next generation of high-performance, energy-efficient training systems.

By introducing energy efficiency as a critical factor in system optimization discussions, we pave the way for more sustainable AI solutions that balance the dual imperatives of performance and environmental responsibility. This holistic approach to the design of the ML system is essential, as we push the limits of AI capabilities while striving to minimize their energy footprint. Our work not only highlights the current challenges in scaling ML training systems, but also sets the stage for innovative solutions that will shape the future of energy-efficient artificial intelligence.

% The time to solution (train) is a key factor in training the ML models.  This is accomplished through various parallel schemes that allow scaling the time to train down with more resources at the same time ensuring that the scaling is meaningful with added resources.  The other aspect of scaling is the energy consumed to train and how it Energy scaling is not linear as you scale up your system (energy increases for same amount of work) - as you increase to higher chip counts you add higher networking, so it expends more energy

% Time to solution (train) is a key factor to train ML models.  This is accomplished through various  parallelization strategies that allow to scale the time to train down with more resources at the same time ensuring that the scaling is meaningful with added resources. Another important consideration is the energy consumption associated with training. Energy scaling does not follow a linear pattern; as you increase to higher chip count, the energy required also rises due to additional networking and infrastructure demands. This means that while adding more resources can reduce training time, it might result in a disproportionate increase in energy usage.

% In this section, we discuss the scalability of training-scale systems from our recently released MLPerf Training power benchmarking. As training systems for ML workloads like LLMs scale for performance [add citation], it is important to consider energy efficiency as another trade-off. Prior work studies trade-offs of optimal scales for performance efficient systems [add citation]. Our work introduces optimal scales for energy efficiency with heavy attention still being spent on performance. 

% However, adding energy as a factor to these system optimization explorations is necessary for next generation systems to facilitate the development of energy-optimized ML processors and accelerators, going beyond mere parallelization for performance scaling. It will also highlight the need to optimize not just compute energy, but also other types of energy consumption, such as interconnect energy.

% \begin{figure}[]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/llama70b_finetune_energy_breakdown.png}
%     \caption{Llama2\_70b\_LoRA Fine Tuning Energy Breakdown}
%     \label{fig:training_energy_breakdown}
% \end{figure}

Figure \ref{fig:training_energy_breakdown} shows the time to training  and energy consumption from our v1.0 training power submissions on llama2-70b, across three different system scales. Energy consumption can be estimated as ( time\_to\_train x (power\_per\_accelerator *number\_of\_accelerator + power\_of\_other\_component)), ideally, with perfect parallelization of workloads, increasing the number of accelerators should proportionally reduce the time to train, leading to linear energy consumption scaling. However, as shown in the figure, because not all parts of the workload can be parallelized there is a diminishing return on the improvement of training time with additional accelerators. Furthermore, as the number of accelerators scales, we must also account for the energy consumed by other components, such as interconnects. Hence in the deployment of future training systems, it is valuable for architects to understand this relationship and consider designing energy efficient accelerators and model level optimizations to improve time to train and hardware efficiency. With more MLPerf Training power data in future submissions and versions, we hope to better define the pareto curves for optimal scales for energy efficiency.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








%show the energy efficiency trends of offline inference data for various workloads over each MLPerf version. The submission with the maximum energy efficiency at each version is normalized to the corresponding workload's earliest version max value. Each version's data is cumulative, meaning that any plotted maximum energy efficiency point can come from any version up to and including the plotted version. The x-axis for every figure labeled by version is spaced by release date, giving a more accurate depiction of trends over time. There will be more in-depth discussion for reasons for the energy efficiency gains and plateaus later in the paper.

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/norm_dc_offline_efficiency_trends.png}
        \caption{Datacenter}
        \label{fig:dc_trends}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/norm_edge_offline_efficiency_trends.png}
        \caption{Edge}
        \label{fig:edge_trends}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tiny_trends.png}
        \caption{Tiny}
        \label{fig:tiny_trends}
    \end{subfigure}
    \caption{Comparison of energy efficiency trends for datacenter, edge, and tiny inference.}
    \label{fig:comparison}
\end{figure*}


% (**** PLEASE FIX IF ANYONE CAN GIVE MORE CONTEXT ON EFFICIENCY PLATEAUS******)
% slope would go down usually if the vendor that submitted the max point from a previous version doesnt submit in subsequent versions

% for more mature networks, people have already found which optimizations work for their hardware so their is not as much room for their improvements, newer networks (gpt) have a lot more room

% \subsubsection{Datacenter @Anirban}

% Figure \ref{fig:dc_trends} shows offline datacenter inference energy efficiency trends. Retinanet shows significant gains from its start in v3.1. Bert-99, ResNet, and RNN-T all show increases in efficiency less than 2x from v1.0. This can indicate that the benchmarked systems are already optimized for these workloads from early on, or because architects fail to direct enough attention to energy efficiency compared to performance. Note that in Figure \ref{fig:mlperf_performance}, performance gains have been steadily achieved at rates above Moore's Law despite the slowdown of transistor scaling. In this paper, we emphasize a call to action to architects to give more attention to energy efficiency when developing the next generations of ML systems. Interestingly, GPT-J achieves a significant gain (***** GIVE SPECIFIC NUMBERS) over its 2 versions of collected data. This can likely be accredited to the significant attention given to LLM computing efficiency due to its significant impact at scale, and we encourage architects to continue this approach across workloads at datacenter scale.


% Figure \ref{fig:edge_trends} shows offline edge inference energy efficiency trends. Like with datacenter, ResNet shows a less than 2x gain from v1.0. While Retinanet, Bert-99.0, and RNN-T workloads all show stronger gains than datacenter early on, they plateau by the last 3 version. Based on magnitudes of gain, especially early on in edge benchmarking, it can be interpreted that significant attention paid to energy efficiency coupled with room to improve created strong gains in edge energy efficiency. However, the plateau's point to a reduction in interest and potential optimizations. With  rapidly growing scales of edge computing implementation, we must put more attention into pushing these energy efficiency curves back on a positive trend.

% The jump for rnnt in v3.1 - a new hardware being submitted?
% The jump for rnnt in v1.1 - ?
% The jump for retinanet in v3.0 - a new hardware being submitted
% Continuous rise for bert-99 until v2.1 - ?
% Plateaus point to no better hardware being submitted in further rounds and also no major software improvements coming (most optimizations already done?)

% Figure \ref{fig:tiny_trends} shows offline tiny inference energy efficiency trends. Although the benchmarks are not comparable with datacenter and edge, note the magnitude of gains on the Y axis of this figure. Compared to the energy efficiency trends shown in the datacenter and edge figures, tiny-scale computing has undergone massive improvements in energy efficiency over its early versions across every workload (between ~100x and ~1000x) and then hit a wall at v1.0. Due to its almost complete novelty at the time MLPerf-Tiny v0.5 was released, tiny computing had significant potential to be optimized at hardware and software levels with relatively straightforward solutions. Now with energy efficiency stagnant over the past 3 versions, we must find more creative ways to continue moving the curves up. While individual tiny electronics consumes magnitudes of power less than datacenter of edge, energy efficiency of these devices is crucial to next generation internet-of-things systems at scale.

% \textbf{Objective}: Discuss improvements in energy efficiency over different generations or iterations of systems.

% \textbf{Why this is good to put in the paper}: Showcasing improvements demonstrates progress and provides benchmarks for future development. This section highlights the impact of various optimizations and advancements in the field.


\subsection{Comparison of Inference ML Systems @Arjun}

At MLCommons, we collect submissions across a wide scale of inference ML systems, ranging from tiny devices consuming power on the order of $\mu$W to datacenter systems on the order of kW. Comparing efficiency, trends, and distributions can give unique insight into energy characteristics of each scale of systems. 

\subsubsection{Datacenter and Edge @Tejus @Arjun}
We visualize relative energy efficiency and submission variability between datacenter and edge data on equivalent workloads in Figures \ref{fig:resnet_variability} and \ref{fig:rnnt_variability}. We have not included tiny because there are no comparable workloads. Each figure represents a workload where the variance indicates the max and min points of all the submissions in a specific category (Red lines are Edge and Blue are datacenter) across the various submissions versions we have had. Datacenter systems are the largest scale MLPerf inference submissions. While Figure \ref{fig:dc_trends} shows that datacenter has the lowest relative energy efficiency improvements compared to Figures \ref{fig:edge_trends} and \ref{fig:tiny_trends}, the unnormalized $\textsf{Samples}/\textsf{Joule}$ from the two variability figures show that depending on a given workload either datacenter or edge system can be better energy efficient. The maximum energy efficiency of the Datacenter points (blue) is higher than the Edge points (red) for every version on the RNN-T. At the same time, the trend is the reverse for ResNet except in v4.0 where the system with the best energy efficiency in the edge category in the previous rounds was not submitted. While a datacenter system typically has more accelerators they typically also have higher idle power. So, even though the idle system power gets amortized by the number of accelerators the energy efficiency of a particular workload can still be lower depending on how well that workload utilizes that given system. 

If we compare the geomeans, datacenter points are always above the edge ones for both ResNet and RNNT. This can attributed to the fact that a lot more ResNet submissions are done in the Edge category (?need to add count) and many of them are not power optimized (off-the-shelf results) pulling the geomean down. Datacenter systems are harder to submit as they require ECC RAM, a more difficult Server scenario etc. and so most of the submissions happen to be optimal performing ones.




\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/resnet_variability.png}
    \caption{ResNet Edge vs. Datacenter Variability, Unnormalized}
    \label{fig:resnet_variability}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/rnnt_variability.png}
    \caption{RNN-T Edge vs. Datacenter Variability, Unnormalized}
    \label{fig:rnnt_variability}
\end{figure}

\subsubsection{Tiny @Jeremy}

\begin{itemize}
    \item Identify the systems tested (e.g., edge devices, datacenters, tiny IoT).
    \item Present metrics used for comparison (e.g., energy per inference, total power consumption).
    \item Highlight significant differences between systems.
    \item Identify factors contributing to efficiency differences (e.g., hardware configurations, workload characteristics).
\end{itemize}

\textbf{Objective}: Compare the energy efficiency of various ML systems (INFERENCE tiny vs edge vs datacenter)

\textbf{Why this is good to put in the paper}: This section provides a comprehensive comparison of different ML systems, highlighting their strengths and weaknesses in terms of energy efficiency. It helps in understanding which systems are more efficient and why, aiding in future design and optimization.

\textbf{Key Points}:
\begin{itemize}
    \item Identify the systems tested (e.g., edge devices, datacenters, tiny IoT).
    \item Present metrics used for comparison (e.g., energy per inference, total power consumption).
    \item Highlight significant differences between systems.
    \item Identify factors contributing to efficiency differences (e.g., hardware configurations, workload characteristics).
\end{itemize}

\subsection{Workload-Specific Insights   @Sachin}


\begin{itemize}
    \item List the workloads analyzed (e.g., image classification, object detection, natural language processing).
    \item Compare energy efficiency across different workloads.
    \item Highlight any patterns or anomalies observed.
    \item Discuss implications for specific application domains.
    \item Include metrics such as energy per user/request for practical relevance.
    \item Compare energy efficiency across different workloads.
\end{itemize}

\textbf{Objective}: 
MLPerf Inference is a benchmark suite designed to measure the performance of machine learning inference across various platforms and applications. It covers a wide range of workloads, including:

\textbf{ Computer Vision }

ResNet-50: A classic image classification model, widely used as a baseline for computer vision tasks.

RetinaNet: An object detection model, designed to identify and locate objects within images.

3D U-Net: A medical image segmentation model, used to segment different structures or regions within medical images.

\textbf{ Natural Language Processing (NLP)}
BERT:** A powerful language model for various NLP tasks, including text classification, question answering, and named entity recognition.

Recommenders 
* **DLRM:** A recommendation model used for predicting user preferences based on historical data.

Speech to Text
* **RNN-T:** A speech recognition model, designed to transcribe spoken language into text.

Generative AI
* **LLM-small:** A smaller language model for natural language understanding and generation tasks.
* **LLM-large:** A larger language model with enhanced capabilities for complex language tasks.
* **Text-to-image:** A model capable of generating images based on text descriptions.


Key Points about MLPerf Inference Workloads
Diverse: Covers a broad spectrum of AI applications, from computer vision to natural language processing and generative AI.

Challenging: Designed to push the limits of hardware and software systems, providing a rigorous benchmark for performance evaluation.

Relevant: Includes representative workloads that reflect real-world use cases in various industries.

Open: The benchmark suite is publicly available, promoting transparency and reproducibility of results.

By evaluating performance on these diverse workloads, MLPerf Inference provides valuable insights into the capabilities of different hardware and software platforms for AI inference.
 

\textbf{Why this is good to put in the paper}: Detailed workload analysis helps in understanding the energy demands of various tasks, providing actionable insights for optimizing specific applications.

\textbf{Key Points}:
\begin{itemize}
    \item Include metrics such as energy per user/request for practical relevance.
    \item Compare energy efficiency across different workloads.
\end{itemize}



%Figure \ref{fig:training_energy_breakdown} shows the energy efficiency from our v1.0 submissions on llama2-70b on 3 different scales of systems. Our measurement of energy efficiency is 1/(latency * energy) in $(min*kJ)^{-1}$, which factors in the square of performance and the raw magnitude of energy efficiency. Note the logarithm-like curve trend between the 3 submission points, indicating positive but diminishing efficiency as the systems scale. This is accredited to (******ADD REASON FOR CURVE SHAPE*****). In deployment of future training systems, it is valuable for architects to understand this relationship and (*****ADD ADVICE/INSIGHTS FOR USAGE*****). With more MLPerf Training power data in future submissions and version, we hope to better define the pareto curves for optimal scales for energy efficiency.


% \begin{itemize}
%     \item Discuss scalability of ML systems from small to large scale (e.g., single node to multi-node clusters).
%     \item Present data on power consumption versus performance metrics (e.g., throughput, latency).
%     \item Analyze trade-offs at different power levels and system scales.
% \end{itemize}

% \textbf{Objective}: Examine how energy efficiency scales with system size and power consumption TRAINING

% \textbf{Why this is good to put in the paper}: Understanding scalability is crucial for deploying ML systems at different scales. This section provides insights into how energy efficiency changes with scale, helping in planning and resource allocation for scalable ML deployments.

% \textbf{Key Points}:
% \begin{itemize}
%     \item Discuss scalability of ML systems from small to large scale (e.g., single node to multi-node clusters).
%     \item Present data on power consumption versus performance metrics (e.g., throughput, latency).
%     \item Analyze trade-offs at different power levels and system scales.
% \end{itemize}


\subsection{Specific Analysis}
As shown in the Energy Efficiency Improvements section, significant gains in efficiency have been seen in the past but are plateauing out in recent MLPerf versions. We break down these improvements by isolating specific sources of efficiency gains, quantifying their magnitude of gains, and understanding their strengths and weaknesses. We aim to give architects and ML engineers more context on sources of energy energy improvement to help drive more informed decisions. Data from this section is from MLPerf Inference Datacenter closed division.

\subsubsection{Hardware-Level Efficiency Improvement Analysis @Yuechao}
\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/tpu_bert.png}
    \caption{Energy Efficiency from Hardware Optimizations. Red: 1/time to train, higher is better; yellow: 1/energy to train, higher is better. \textbf{Remove perf/power, and change power score to 1/power score}}
    \label{fig:hardware_improvement}
\end{figure}

ML processor architectures are becoming more efficient by focusing on optimizing instruction sets, utilizing specialized cores for different tasks, and employing techniques like pipelining and out-of-order execution. This allows for more work to be done in a single clock cycle, reducing the need for constant high clock speeds. 

In Figure \ref{fig:hardware_improvement}, we evaluate a case study on hardware optimizations where we use similar hardware scale, lock the software stack including quantization, and evaluate subsequent versions of a neural network ASIC on the BERT workload. We see a general trend across the hardware versions in reduction in both time and energy to train. 

% \sout{Multiplying these optimizations to calculate energy efficiency (blue bar) shows steep increases.}

% \sout{While it is well explored that hardware optimization can be traded for workload generalizability, our evaluation shows that there is still significant room for energy efficiency improvements while preserving capabilities. (***talk about strengths/weaknesses and how to use***) - Not covered in text and I don't think we have data to support this.}

The computing units in newer ML accelerators generally have features yielding better energy efficiency: supports of lower numeric precision, more efficient designs for the same precision, and better handling of memory-compute coordination. We also see significant improvements in the fast inter-connects between ML accelerators in terms of higher bandwidth, lower latency and supports of more diverse communication patterns. Hardware / Cloud providers attend to make the migration to newer accelerators as smooth as possible, so that their users can leverage the benefits of hardware advancement, of which better energy efficiency being an important one. There are also potential changes on the user side that can reduce the cost to complete the same ML task: higher per-accelerator batch sizes to better utilize the RAM of accelerators or to reduce the accelerator scale, lower precision / quantization to reduce both compute and memory requirements, etc.

% \sout{@Yuechao more context on software stack across TPU versions in graph? more insight into how people can apply this info to their work? Maybe give some qualitative insight into different components (e.g., hardware accelerators, memory hierarchies, host CPU, interconnects). - See the paragraph before.}

Also, although not quantitatively evaluated, power management techniques like dynamic voltage and frequency scaling (DVFS) allow processors to adjust their power consumption based on workload demands. When processing simpler tasks, the system can lower its clock speed and voltage, reducing power usage.


% \begin{itemize}
%     \item Present before-and-after scenarios to show the impact of these optimizations.
%     \item Discuss the role of software, hardware, and quantization techniques in improving efficiency.
%     \item Describe the configurations tested (e.g., hardware accelerators, memory hierarchies, interconnects).
%     \item Present data on how these configurations affect energy efficiency.
%     \item Discuss implications for designing energy-efficient systems.
%     \item Include insights into host, CPU, and network contributions to the overall energy efficiency.
%     \item Discuss the interplay between different components and their collective impact on efficiency.
% \end{itemize}

% \textbf{Objective}: Detail specific optimizations (software, hardware, quantization) that led to efficiency improvements.

% \textbf{Why this is good to put in the paper}: Highlighting specific optimizations shows the practical steps taken to achieve energy efficiency, providing a roadmap for future efforts in the field.

% \textbf{Key Points}:
% \begin{itemize}
%     \item Present before-and-after scenarios to show the impact of these optimizations.
%     \item Discuss the role of software, hardware, and quantization techniques in improving efficiency.
% \end{itemize}

\subsubsection{Software-Level Efficiency Improvement Analysis @Miro}


With each generation of submissions, software techniques have been deployed to improve on the bottlenecks to speedup the time taken for inference or  the iteration time in training. In many instances, reducing the time comes from optimizations that reduce energy consumed, an example would be to make the work being done from layer to layer of a network to be resident on the chip to limit the power consumed in DRAM and in addition it speeds up the time to do the work since on chip memory is faster and more energy efficient.

In Figure \ref{fig:software_histogram}, we identify submissions with the same hardware configurations (host CPU, number of accelerators, type of accelerators) on 2 adjacent versions of any workload. We see that ~89\% of the data in the histogram is positive, indicating that most submissions on comparable hardware show some magnitude software-level efficiency improvements. We hypothesize that the small amount of data exhibiting a low decrease in efficiency may be due to changes in configurations not accounted for by our equivalent hardware comparison or vendor changes not addressing energy efficiency. It is equally important to note that 18\% of the data achieves over 50\% energy efficiency gains, which shows strong historical evidence that software optimizations have contributed to energy efficient systems.

We evaluate a similar case study on software optimizations where we identify comparable systems across 4 versions of ResNet workloads. While performance (red bar) reduces slightly, power consumption (yellow bar) reduces at a more rapid rate leading to improved energy efficiency (blue bar). Further exploration into these submissions indicate that optimizations to the software development kits (SDK) and total cost of ownership (TCO) contribute to the energy efficiency improvements. Sacrificing a small magnitude of performance for these software-level optimization additions achieves significant energy efficiency gains.

**MORE CONTEXT, OTHER SOURCES, HOW TO USE?***


\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/software_histogram.png}
    \caption{Energy Efficiency from Software Optimizations Deltas Histogram}
    \label{fig:software_improvement}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/software_opt.png}
    \caption{Energy Efficiency from Software Optimizations}
    \label{fig:software_histogram}
\end{figure}

\subsubsection{Low Precision Efficiency Improvement Analysis}

Quantization inherently improves performance and power consumption by using less computation, either explicitly or through improved parallelism. However, because MLPerf benchmarks require submissions to achieve a minimum accuracy, submitters must make informed decisions to use more aggressive quantization to improve performance and energy efficiency while still meeting the accuracy target. In Figure \ref{fig:quant_improvement}, we compare the power efficiency of systems on the Bert-99 (blue bar) and Bert-99.9 (orange bar) workload. The BERT-99 (low accuracy) benchmark requires the submission to meet 99\% of the original single precision floating point (FP32) model's accuracy, while for BERT-99.9 (high accuracy), the threshold is set to 99.9\% of FP32 accuracy. The data is normalized to the Bert-99 (low accuracy) performance/Watt (perf/W) at each version or MLPerf-Inference.  Each cluster in the chart compares the relative perf/W between the BERT-99 and BERT-99.9 (offline, datacenter) submissions on the same hardware platform in the same version of MLPerf-Inference. Each Bert-99 submission uses INT8 quantization since INT8 is sufficient to meet the 99\% accuracy target, but cannot meet the higher accuracy target of the BERT-99.9 benchmark. For BERT-99.9, submitters needed 16-bit floating point (FP16) to meet the accuracy target until v3.1, where new hardware with 8-bit floating point (FP8) formats enabled higher performance and power efficiency while still meeting the 99.9\% accuracy target. As a result, the perf/W of the BERT-99.9 submissions jumped from ~50\% of BERT-99 in older submissions to ~85\% of BERT-99. The lower precision floating point format consumes lower energy per op in computing the matrix multiplication as well as lower energy in effective data moved in the memory subsystem resulting in the gains observed.



\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/bert_quantization_2.png}
    \caption{Energy Efficiency from Quantization Optimizations}
    \label{fig:quant_improvement}
\end{figure}

% \section{Discussion @VJ @Arya}

% Trying to balance adaptability with accuracy
% Develop a super accurate methodology, but if one submitter submits as compared to having a more broader or more relax method that allows for more people to participate
% Limitations
% Lack of common read out interfaces, between different vendors and CSPs
% Not all the systems communicate in the same way, so we can’t develop a common framework
% Large scale datacenter is also hard to measure, therefore decisions were made a certain way
% There is an inherent limitation with respect to hardware scalability
% Only way to move forward is software based methods, to get around hardware analyzers everywhere 
% Lessons about power measurement and how you do it
% Case study / example

\subsection{Accuracy-Level Efficiency Improvement}

Datacenter/Edge histogram (99.9 sam/j)/(99.0 sam/j) where number less than 1 means that there is an efficiency degredation with higher accuracy and 1 means they just resubmitted
